Shortest-Path Flow Matching with Mixture-Conditioned Bases for OOD Generalization to Unseen Conditions

Robust generalization under distribution shift remains a key challenge for conditional generative modeling: conditional flow-based methods often fit the training conditions well but fail to extrapolate to unseen ones. We introduce SP-FM, a shortest-path flow-matching framework that improves out-of-distribution (OOD) generalization by conditioning both the base distribution and the flow field on the condition. Specifically, SP-FM learns a condition-dependent base distribution parameterized as a flexible, learnable mixture, together with a condition-dependent vector field trained via shortest-path flow matching. Conditioning the base allows the model to adapt its starting distribution across conditions, enabling smooth interpolation and more reliable extrapolation beyond the observed training range. We provide theoretical insights into the resulting conditional transport and show how mixture-conditioned bases enhance robustness under shift. Empirically, SP-FM is effective across heterogeneous domains, including predicting responses to unseen perturbations in single-cell transcriptomics and modeling treatment effects in high-content microscopy--based drug screening. Overall, SP-FM provides a simple yet effective plug-in strategy for improving conditional generative modeling and OOD generalization across diverse domains.

==> history/MixFlow_arXiv/4_generalisation_OLD.tex <==
\section{Generalization Analysis}
\label{sec:generalization}

We analyze why mixture-conditioned flow matching improves generalization to unseen descriptors. 
Our focus is the initial velocity field $v_\theta(\cdot,0;\myvect y)$, which sets the starting direction of the flow from the conditional base $q_{w(\myvect y)}$ toward the target $\rho(\cdot\mid\myvect y)$. 
Throughout, we use an \emph{idealized teacher} for clarity and later discuss the practical implications.

\paragraph{Idealized teacher and objective.}
For descriptor $\myvect y$, let $w(\myvect y)=h_\phi(\myvect y)\in\Delta^{K-1}$ be the predicted mixture weights and 
$q_{w(\myvect y)}=\sum_{k=1}^K w_k(\myvect y)\,\mathcal{N}(\mu_k,\Sigma_k)$ the conditional base.
Let $T_{\myvect y}$ denote the Brenier optimal transport map from $q_{w(\myvect y)}$ to $\rho(\cdot\mid\myvect y)$, and define the (ideal) displacement field
\begin{equation}
u_{\myvect y}(x) \;=\; T_{\myvect y}(x)-x, \qquad x\sim q_{w(\myvect y)}.
\end{equation}
Training with a $W_2$–geodesic teacher amounts to regressing $v_\theta(\cdot,0;\myvect y)$ to $u_{\myvect y}(\cdot)$ under samples $x\sim q_{w(\myvect y)}$. 
For analysis, we additionally consider the alignment of the base by the auxiliary objective
\begin{equation}
\label{eq:aux-w2}
w(\myvect y)\;\in\;\argmin_{w\in\Delta^{K-1}} \; W_2^2\!\big(q_w,\;\rho(\cdot\mid\myvect y)\big),
\end{equation}
which captures the fact that sampling $x_0\sim q_{w(\myvect y)}$ and using a $W_2$ teacher nudges $h_\phi$ toward weights that better align $q_{w(\myvect y)}$ with $\rho(\cdot\mid\myvect y)$.\footnote{In practice, $h_\phi$ is trained through the flow-matching loss, not by directly minimizing~\eqref{eq:aux-w2}; the auxiliary objective is a standard device to make the analysis precise.}

\paragraph{Weight–redistribution tangent space.}
Consider infinitesimal reweightings $w(\epsilon)=w+\epsilon\,\delta w$ with $\sum_k \delta w_k=0$. 
Let $\Phi_k$ denote the $W_2$ first-variation potentials associated with changing the $k$-th weight (formally defined via the dual of~\eqref{eq:aux-w2}). 
First-order optimality of~\eqref{eq:aux-w2} implies the $L^2(q_{w(\myvect y)})$ orthogonality conditions
\begin{equation}
\label{eq:l2-orth}
\int_{\R^D} u_{\myvect y}(x)\cdot\nabla \Phi_k(x)\; q_{w(\myvect y)}(x)\,dx \;=\; 0,
\qquad k=1,\dots,K-1,
\end{equation}
i.e., $u_{\myvect y}$ lies in the orthogonal complement of the \emph{weight–redistribution tangent space} spanned by $\{\nabla\Phi_k\}_{k=1}^{K-1}$ in $L^2(q_{w(\myvect y)})$.
Intuitively, directions that merely \emph{reshuffle mixture weights} are suppressed at $t=0$.

\paragraph{From function space to a finite-dimensional subspace.}
To obtain a concrete geometric picture, we specialize to a common regime.

\begin{assumption}[Well-separated, near-isotropic components]
\label{asmp:isotropic}
Each component is (approximately) isotropic, $\Sigma_k\approx \sigma_k^2 I$, and components are well-separated so that responsibilities are nearly one-hot in regions of high density for each component.
Moreover, $u_{\myvect y}(x)$ varies slowly within a component support.
\end{assumption}

Under Assumption~\ref{asmp:isotropic}, reweighting primarily shifts the base mean along directions spanned by $\{\mu_k-\mu_{K}\}_{k=1}^{K-1}$. 
Then~\eqref{eq:l2-orth} reduces to (component-averaged) orthogonality with respect to those mean-shift directions. 
In the vanishing-covariance limit this becomes pointwise:
\begin{equation}
\label{eq:ptwise-orth}
u_{\myvect y}(x)\;\perp\; \mathrm{span}\{\mu_1-\mu_K,\;\mu_2-\mu_K,\;\dots,\;\mu_{K-1}-\mu_K\}
\quad \text{for $q_{w(\myvect y)}$-a.e.\ $x$.}
\end{equation}
Define the effective subspace dimension
\begin{equation}
\label{eq:deff}
d_{\mathrm{eff}} \;=\; D \;-\; \mathrm{rank}\{\mu_k-\mu_K : k=1,\dots,K-1\}.
\end{equation}
Thus, the mixture base induces $K{-}1$ orthogonality constraints (up to rank), shrinking the admissible set of initial directions $u_{\myvect y}$ to a $d_{\mathrm{eff}}$-dimensional subspace of $\R^D$.

\paragraph{Implications for generalization (informal).}
Let $\mathbf{V}$ be the function class used to parameterize $v_\theta(\cdot,0;\myvect y)$ (e.g., a linear-in-parameters velocity network at $t=0$).
Since training regresses onto $u_{\myvect y}$ under the constraints~\eqref{eq:l2-orth}–\eqref{eq:ptwise-orth}, the \emph{relevant} hypothesis class is the projection $P_\perp \mathbf{V}$ onto the orthogonal complement of the weight–redistribution span. 
For standard linear classes with bounded norm, the empirical Rademacher complexity satisfies
\begin{equation}
\label{eq:rademacher}
\mathfrak R\big(P_\perp \mathbf{V}\big)
\;\;\lesssim\;\;
\sqrt{\frac{d_{\mathrm{eff}}}{N}}
\quad\text{(up to problem-dependent constants),}
\end{equation}
where $N$ is the number of training populations and $d_{\mathrm{eff}}$ is given by~\eqref{eq:deff}. 
Equation~\eqref{eq:rademacher} should be viewed as a \emph{scaling law}: orthogonality constraints reduce the effective dimension of $v_\theta(\cdot,0;\myvect y)$, tightening generalization bounds relative to conditioning that learns population-specific estimators.

\paragraph{Bias--variance tradeoff in $K$.}
Increasing $K$ enlarges the $\mathrm{span}\{\mu_k-\mu_K\}$ (non-decreasing rank), which \emph{reduces} $d_{\mathrm{eff}}$ and hence the variance term suggested by~\eqref{eq:rademacher}.
At the same time, a richer mixture family tightens the approximation of $\rho(\cdot\mid\myvect y)$ by $q_{w(\myvect y)}$ (lower bias in the teacher alignment).
Thus $K$ controls a bias--variance tradeoff: larger $K$ yields stronger structural constraints at $t=0$ \emph{and} a better-aligned base, which together improve OOD performance until finite-sample or optimization limits dominate.\footnote{If component means are themselves low-rank (e.g., lie near a manifold), the realized gain saturates once $\mathrm{rank}\{\mu_k-\mu_K\}$ plateaus. If components differ mainly in covariance rather than mean, analogous constraints emerge along principal covariance-change directions (see App.~\ref{app:proofs}).}

\paragraph{Practical takeaway.}
Mixture-conditioning does not merely add parameters; it imposes \emph{structural} $t{=}0$ constraints that suppress weight-redistribution directions and concentrate learning capacity on biologically relevant displacements. 
This ``capacity focusing'' effect explains why MixFlow generalizes to unseen perturbations better than conditioning schemes that effectively train independent estimators per population.

\paragraph{Relation to the training objective.}
While we analyze an idealized $W_2$ teacher and the auxiliary alignment~\eqref{eq:aux-w2}, the same constraints qualitatively arise whenever (i) $x_0$ is drawn from $q_{w(\myvect y)}$, (ii) the teacher couples $x_0$ to target samples via displacement-like supervision, and (iii) gradients backpropagate through $h_\phi$ (e.g., via reparameterization or low-variance estimators). 
Under these conditions, $h_\phi$ is driven to reduce transport along weight-redistribution directions, yielding the same subspace effect at $t{=}0$.

\paragraph{Proof sketches (moved to Appendix).}
We provide details in App.~\ref{app:proofs}.
\begin{itemize}
\item \textbf{Lemma A.1 (First-order conditions).} Derives~\eqref{eq:l2-orth} from the dual of~\eqref{eq:aux-w2} using the envelope theorem and properties of $W_2$ barycenters.
\item \textbf{Proposition A.2 (Mean-shift reduction).} Under Assumption~\ref{asmp:isotropic}, shows that $\{\nabla\Phi_k\}$ align with mean-shift directions, yielding~\eqref{eq:ptwise-orth} in the small-variance limit.
\item \textbf{Lemma A.3 (Projected complexity).} For linear-in-parameters velocity classes with bounded norm, proves the scaling in~\eqref{eq:rademacher} after projection by $P_\perp$.
\end{itemize}

